DART: Diversify-Aggregate-Repeat Training Improves Generalization of Neural Networks

Generalization of neural networks is crucial for deploying them safely in the real world. Common training strategies to improve generalization involve the use of data augmentations, ensembling and model averaging. In this work, we first establish a surprisingly simple but strong benchmark for generalization which utilizes diverse augmentations within a training minibatch, and show that this can learn a more balanced distribution of features. Further, we propose Diversify-Aggregate-Repeat Training (DART) strategy that first trains diverse models using different augmentations (or domains) to explore the loss basin, and further Aggregates their weights to combine their expertise and obtain improved generalization. We find that Repeating the step of Aggregation throughout training improves the overall optimization trajectory and also ensures that the individual models have a sufficiently low loss barrier to obtain improved generalization on combining them. We shed light on our approach by casting it in the framework proposed by Shen et al. and theoretically show that it indeed generalizes better. In addition to improvements in In- Domain generalization, we demonstrate SOTA performance on the Domain Generalization benchmarks in the popular DomainBed framework as well. Our method is generic and can easily be integrated with several base training algorithms to achieve performance gains.

==> tables/OOD.tex <==
\begin{table}
\caption{\textbf{OOD Performance:} Performance (\%) of DART using Pad+Crop+HFlip (PCH) augmentations across all branches, when compared to ERM training, on the corruptions datasets CIFAR10-C and CIFAR100-C using WideResNet-28-10 model. Standard deviation is reported across 5 reruns}
\vspace{-0.15cm}
\centering
\setlength\tabcolsep{2pt}
\resizebox{1.0\linewidth}{!}{
\label{table:ood_updated}
\begin{tabular}{lcccc}
\toprule
Method & CIFAR-10 & CIFAR10-C & CIFAR-100 & CIFAR100-C    
     \\
\midrule
ERM+EMA (PCH)	& 96.41 \std{0.13} & 77.56 \std{0.15} & 81.67 \std{0.08} & 54.22 \std{0.11} \\
DART (Ours, PCH) & \textbf{96.64} \std{0.11} & \textbf{78.25} \std{0.17} & \textbf{82.31} \std{0.18} & \textbf{55.05} \std{0.13} \\
\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\end{table}

==> tables/ablations.tex <==
\begin{table}
\caption{\textbf{Ablation experiments on CIFAR10 and CIFAR100:} Performance (\%) of the proposed method with different variations in the training algorithm. Variance is reported over 3 reruns, except for DART (A0) whose variance is reported over 5 reruns.}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\label{table:ablation}
\begin{tabular}{lcc}
\toprule
Method & CIFAR-10 & CIFAR-100    \\
\midrule
\textbf{A0} First-half common training  (DART)        & 97.96 \std{0.06}                                                        & 86.46 \std{0.12}           \\
\textbf{A4} Train experts after 500 epochs of common                            & 97.85 \std{0.05}                                                        & 85.91 \std{0.15}   \\
~~~~~~training  (no intermediate interpolations) &     &     \\
\textbf{A5} Train experts after 550 epochs of common                              & 97.76 \std{0.11}                                                        & 85.58 \std{0.25}    \\
~~~~~~training (no intermediate interpolations) & & \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/miro.tex <==
\begin{table}
\vspace{-0.3cm}
\caption{\textbf{Integrating DART with MIRO and SWAD:} OOD performance (\%) on OfficeHome of the
proposed method DART coupled with MIRO \cite{cha2022miro} and SWAD \cite{cha2021swad} on different pretrained backbones. }
\vspace{-0.1cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\label{table:miro}
\begin{tabular}{ccccc}
\toprule

                                    \textbf{MIRO} & \textbf{MIRO+SWAD} & \textbf{~~DART~~} & \textbf{DART+MIRO} & \textbf{DART+MIRO+SWAD} \\
                                   \midrule
 83.35         & 84.80              & 80.98         & 86.14              & \textbf{87.37}  \\

\bottomrule
\end{tabular}
\vspace{-0.1cm}
}
\end{table}
